Multimodal normative modeling in Alzheimers Disease with introspective variational autoencoders

Normative modeling learns a healthy reference distribution and quantifies subject-specific deviations to capture heterogeneous disease effects. In Alzheimers disease (AD), multimodal neuroimaging offers complementary signals but VAE-based normative models often (i) fit the healthy reference distribution imperfectly, inflating false positives, and (ii) use posterior aggregation (e.g., PoE/MoE) that can yield weak multimodal fusion in the shared latent space. We propose mmSIVAE, a multimodal soft-introspective variational autoencoder combined with Mixture-of-Product-of-Experts (MOPOE) aggregation to improve reference fidelity and multimodal integration. We compute deviation scores in latent space and feature space as distances from the learned healthy distributions, and map statistically significant latent deviations to regional abnormalities for interpretability. On ADNI MRI regional volumes and amyloid PET SUVR, mmSIVAE improves reconstruction on held-out controls and produces more discriminative deviation scores for outlier detection than VAE baselines, with higher likelihood ratios and clearer separation between control and AD-spectrum cohorts. Deviation maps highlight region-level patterns aligned with established AD-related changes. More broadly, our results highlight the importance of training objectives that prioritize reference-distribution fidelity and robust multimodal posterior aggregation for normative modeling, with implications for deviation-based analysis across multimodal clinical data.

==> Figures_tables/cog_correlation_table.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \caption{Pearson correlation coefficients to show the correlation between $D_{ml}$ of different methods with the neuropsychological composites : memory, executive, language and visual-spatial. The numbers in () represent the Steiger's Z-test \cite{steiger1980tests} p values to compare the correlations between mmSIVAE and the baselines. p-values more than 0.05 (marked in red) indicate that the differences are not significant. For fair comparison, all multimodal methods used MOPOE aggregation.}
% \label{tab:cog_correlation_table}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}|l|cccc|@{}}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{1}{c|}{Memory} & \multicolumn{1}{c|}{Executive} & \multicolumn{1}{c|}{Language} & Visual-spatial \\ \cmidrule(l){2-5} 
%                         & \multicolumn{4}{c|}{Pearson correlation coefficient   (Sigel’s Z-test p-value)}                               \\ \midrule
% Multimodal introVAE     & \multicolumn{1}{c|}{-0.573} & \multicolumn{1}{c|}{-0.467}    & \multicolumn{1}{c|}{-0.421}   & -0.442         \\ \midrule
% Unimodal introVAE – concat (MRI + amyloid) &
%   \multicolumn{1}{c|}{-0.521 (\textcolor{red}{0.304})} &
%   \multicolumn{1}{c|}{-0.472 (\textcolor{red}{0.903})} &
%   \multicolumn{1}{c|}{-0.375 (\textcolor{red}{0.064})} &
%   -0.326 (0.032) \\ \midrule
% Multimodal VAE &
%   \multicolumn{1}{c|}{-0.423 (0.0087)} &
%   \multicolumn{1}{c|}{-0.385 (0.027)} &
%   \multicolumn{1}{c|}{-0.392 (\textcolor{red}{0.174})} &
%   -0.294 (0.011) \\ \midrule
% Unimodal VAE – concat (MRI + amyloid) &
%   \multicolumn{1}{c|}{-0.394 (0.0023)} &
%   \multicolumn{1}{c|}{-0.402 (\textcolor{red}{0.074})} &
%   \multicolumn{1}{c|}{-0.374 (\textcolor{red}{0.071})} &
%   -0.306 (0.018) \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!htbp]
\caption{Pearson correlation coefficients between latent deviation $D_{ml}$ and neuropsychological composite scores (memory, executive, language, visual--spatial). Values in parentheses denote Steiger's Z-test $p$-values \cite{steiger1980tests} comparing each method against mmSIVAE. $p$-values $>0.05$ (marked in red) indicate non-significant differences. All multimodal methods use MOPOE aggregation.}
\label{tab:cog_correlation_table}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l c c c c}
\toprule
\textbf{Method} & \textbf{Memory} & \textbf{Executive} & \textbf{Language} & \textbf{Visual-spatial} \\
\midrule

\textbf{mmSIVAE} 
& -0.573 
& -0.467 
& -0.421 
& -0.442 \\

\addlinespace
Unimodal SIVAE (MRI + amyloid)
& -0.521 (\textcolor{red}{0.304})
& -0.472 (\textcolor{red}{0.903})
& -0.375 (\textcolor{red}{0.064})
& -0.326 (0.032) \\

Multimodal VAE
& -0.423 (0.0087)
& -0.385 (0.027)
& -0.392 (\textcolor{red}{0.174})
& -0.294 (0.011) \\

Unimodal VAE (MRI + amyloid)
& -0.394 (0.0023)
& -0.402 (\textcolor{red}{0.074})
& -0.374 (\textcolor{red}{0.071})
& -0.306 (0.018) \\

\bottomrule
\end{tabular}
\end{table*}


==> Figures_tables/outlier_detection.tex <==
\begin{figure*}[!htbp]
  \centering
  % \begin{minipage}[t]{0.49\linewidth}\vspace{0pt}
  %   \centering
  %   \includegraphics[width=\linewidth]{Plots_tables/125k_age.pdf}
  % \end{minipage}\hfill
  \begin{minipage}[t]{0.49\linewidth}\vspace{0pt}
    %\caption*{Likelihood ratio corresponding to outliers derived from $D_{ml}$ for different latent dimensions d = 5, 10, 15 and 20. Higher likelihood ratio indicate better detection of outlier AD patients.}
    \centering
    \scriptsize
    \begin{tabular}{l c c c c}
    \toprule
    \textbf{Method} & \textbf{$d=5$} & \textbf{$d=10$} & \textbf{$d=15$} & \textbf{$d=20$} \\
    \midrule
    
    \textbf{mmSIVAE} & & & & \\
    \quad MOPOE & 7.21 & 7.85 & \textbf{10.2} & 9.34 \\
    \quad POE   & 7.05 & 6.82 & 7.86 & 8.10 \\
    \quad MOE   & 7.21 & 7.85 & 9.21 & 8.56 \\
    \addlinespace
    
    \textbf{mmVAE} & & & & \\
    \quad MOPOE & 6.73 & \textbf{8.10} & 5.72 & 4.56 \\
    \quad MOE   & 6.26 & 7.57 & 5.45 & 5.68 \\
    \quad POE   & 6.21 & 7.95 & 5.68 & 4.89 \\
    \addlinespace
    
    \textbf{Unimodal baselines} & & & & \\
    \quad SIVAE (MRI+Amy) & 4.91 & 5.86 & 7.43 & 6.90 \\
    \quad SIVAE (MRI)     & 7.22 & 6.85 & 8.56 & 8.25 \\
    \quad SIVAE (Amy)     & 7.25 & 6.82 & 8.41 & 8.83 \\
    \quad mmJSD           & 6.31 & 7.21 & 4.66 & 5.25 \\
    \quad JMVAE           & 5.68 & 7.85 & 5.10 & 4.51 \\
    \quad MVTCAE          & 6.34 & 6.83 & 5.56 & 3.82 \\
    
    \bottomrule
    \end{tabular}
  \end{minipage}\hfill
    \begin{minipage}[t]{0.49\linewidth}\vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{Figures_tables/feature_mahalanobis_histogram.pdf}
    %\caption*{Histograms showing the distribution of feature mahalanobis deviations $D_{mf}$ (Equation \ref{d_mf}) for the test (AD patients) and a holdout healthy control cohort. The values in the caption of each subfigure indicate the Earth mover's distance between the 2 distributions train and test. Higher distance indicate lesser overlap and better separation between the control and disease cohorts.}
  \end{minipage}
  \caption{\textbf{A} Likelihood ratio corresponding to outliers derived from $D_{ml}$ for different latent dimensions d = 5, 10, 15 and 20. \textit{Higher likelihood ratio indicate better detection of outlier AD patients.} \textbf{B} Histograms showing the distribution of feature mahalanobis deviations $D_{mf}$ (Equation \ref{d_mf}) for the test (AD patients) and a holdout healthy control cohort. The values in the caption of each subfigure indicate the Earth mover's distance between the 2 distributions train and test. \textit{Higher distance indicate lesser overlap and better separation between the control and disease cohorts.}}
  \label{fig:outlier_detection}
  \vspace{-10pt}
\end{figure*}

==> Sections/background.tex <==
Let $X=\{x_1,\ldots,x_N\}$ denote a set of $N$ modalities (e.g., MRI- and PET-derived regional features) generated from a shared latent variable $z$. A multimodal variational autoencoder (mVAE) specifies the generative model $p_\theta(X,z)=p(z)\prod_{i=1}^{N}p_\theta(x_i\mid z)$ with prior $p(z)$. Given an approximate joint posterior $q_\phi(z\mid X)$, the evidence lower bound (ELBO) is $\operatorname{ELBO} = \mathbb{E}_{q(z \mid X)}\left[\sum_{x_i \in X} \log p_\theta\left(x_i|z\right)\right]-  \operatorname{KL}\left[q_\phi(z|X),p(z)\right]$.

\subsection{Soft-Introspective VAE (SIVAE)}

\paragraph{Introspective VAE:} Unlike the standard VAE, which optimizes a single lower bound, Introspective VAE (IntroVAE) (\cite{huang2018introvae}) incorporates an adversarial learning strategy similar to that used in Generative Adversarial Networks (GANs). In this framework, the encoder's objective is to maximize the KL divergence between the generated (fake) image and the latent variable while minimizing the KL divergence between the actual image and the latent variable. 
$\mathcal{L}_E=ELBO(x)+\sum_{s=r, g}\left[m-KL\left(q_\phi\left(z \mid x_s\right) \| p(z)\right]]\right.$, where $x_r$ is the reconstructed image, $xg$ is the generated image, and $m$ is the hard threshold for constraining the KL divergence. 

Simultaneously, the decoder seeks to challenge the encoder by minimizing the KL divergence between the generated image and the latent variable. 
\vspace{-5mm}
\begin{equation}
\mathcal{L}_D= ELBO(x) + \sum_{s=r, g}\left[K L\left(q_\phi\left(z \mid x_s\right) \| p(z)\right)\right]
\end{equation}
\vspace{-5mm}
% $\mathcal{L}_D= ELBO(x) + \sum_{s=r, g}\left[K L\left(q_\phi\left(z \mid x_s\right) \| p(z)\right)\right]$ 

\paragraph{Soft-Introspective VAE:} A key limitation of IntroVAE is its use of a hard threshold m to constrain the KL divergence term. Soft-Introspective VAE (SIVAE; \cite{daniel2021soft}) argue that this design significantly reduces the model's capacity and can lead to vanishing gradients. To address this issue, SIVAE proposes utilizing the entire Evidence Lower Bound (ELBO) rather than just the KL divergence, employing a soft exponential function in place of a hard threshold. The learning objective (i.e., loss function) for SIVAE is as follows:

\noindent $\mathcal{L}_{E_\phi}(x, z)=E L B O(x)-\frac{1}{\alpha} \exp \left(\alpha E L B O\left(D_\theta(z)\right)\right) \\
\mathcal{L}_{D_\theta}(x, z)=E L B O(x)+\gamma E L B O\left(D_\theta(z)\right)$

% \vspace{-5mm}
% \begin{equation*}
% \begin{aligned}
% & \mathcal{L}_{E_\phi}(x, z)=E L B O(x)-\frac{1}{\alpha} \exp \left(\alpha E L B O\left(D_\theta(z)\right)\right) \\
% & \mathcal{L}_{D_\theta}(x, z)=E L B O(x)+\gamma E L B O\left(D_\theta(z)\right) \label{SIVAE}
% \end{aligned}
% \end{equation*}
% \vspace{-5mm}

\subsection{Approximating joint posterior in the latent space}

Two commonly used strategies for multimodal posterior aggregation are Product-of-Experts (PoE) and Mixture-of-Experts (MoE).
PoE defines
$q_{\mathrm{PoE}}(z|X)\propto p(z)\prod_{i=1}^{N} q_\phi(z|x_i)$,
which can produce a sharp joint posterior but may be dominated by a highly precise or miscalibrated modality, thereby suppressing complementary information from weaker modalities and leading to brittle inference \cite{wu_multimodal_2018}.

MoE averages unimodal posteriors,
$q_{\mathrm{MoE}}(z|X)=\tfrac{1}{N}\sum_{i=1}^{N} q_\phi(z|x_i)$,
with corresponding ELBO \\
$\mathcal{L}_\mathrm{MoE}(X) = \mathbb{E}{q_{\mathrm{MoE}}(z|X)}
\Big[\sum_{i=1}^{N}\log p_\theta(x_i|z)\Big] - \mathrm{KL}\left(q_{\mathrm{MoE}}(z|X),|,p(z)\right)$.
By reducing reliance on any single expert, MoE improves robustness but often yields a joint posterior that is no sharper than the unimodal posteriors, limiting the effectiveness of the shared latent representation for downstream deviation detection \cite{shi2019variational}


==> Sections/discussion.tex <==
% \section{Discussion}
% \label{sec:discussion}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% This work proposes mmSIVAE, a multimodal soft-introspective VAE for normative modeling, together with MOPOE aggregation for constructing an informative joint posterior.
% Across experiments, mmSIVAE improves (i) reconstruction fidelity on held-out healthy controls (Fig.~\ref{fig:recon_comparison_Aim3}), (ii) separation between healthy and AD-spectrum cohorts using both latent- and feature-based deviation scores (Table~\ref{tab:latent_sig_ratio_table}; Fig.~\ref{fig:feature_mahalanobis_histogram}), (iii) association of deviation scores with cognitive composites (Table~\ref{tab:cog_correlation_table}), and (iv) interpretability via region-level deviation maps across clinical stages (Fig.~\ref{fig:effect_size_interpretability}).

% \paragraph{Why soft-introspective training helps normative modeling.}
% Normative modeling places a premium on accurately modeling the reference distribution; if a model reconstructs healthy controls poorly, reconstruction-based deviation scores can inflate false positives and degrade outlier separation.
% The soft-introspective objective \cite{daniel2021soft} introduces an encoder--decoder game that explicitly discourages generated samples from being mapped close to the prior while maintaining good reconstructions for real samples, which can sharpen the learned representation of the reference distribution.
% In our setting, this improved fidelity is reflected in reduced reconstruction errors on held-out healthy controls and in downstream deviation-score separability.

% \paragraph{Why MOPOE improves multimodal deviation scoring.}
% Multimodal posterior aggregation strongly influences whether the shared latent captures complementary information across modalities.
% PoE can be brittle when one modality becomes overconfident, suppressing evidence from the other modality \cite{wu_multimodal_2018}, while MoE can under-fuse modalities, yielding a joint representation that is not substantially more informative than unimodal posteriors \cite{shi2019variational}.
% MOPOE mixes PoE posteriors across modality subsets, balancing sharpness with robustness; empirically, this yields more discriminative latent deviations and better separation between healthy and AD-spectrum cohorts.
% This is particularly important for normative modeling, where deviation scores derived from the latent space depend on a well-calibrated joint posterior.

% \paragraph{Clinical meaning and intended use.}
% The proposed deviation scores are intended to support research on disease heterogeneity, stratification, and hypothesis generation rather than to serve as a standalone diagnostic tool.
% Associations with cognitive composites suggest that the learned deviations capture clinically meaningful variation beyond coarse group labels, and region-level deviation maps provide a complementary interpretation of where abnormalities arise across modalities.
% However, any clinical use would require prospective validation, calibration, and evaluation of reliability across sites and populations.

% \paragraph{Limitations and Future directions}
% First, results are demonstrated on ADNI, and generalization may be affected by site, scanner, or demographic differences; broader validation is required.
% Second, our deviation scores rely on Gaussian modeling of latent embeddings and reconstruction errors; covariance estimation and potential regularization choices can influence Mahalanobis distances, particularly in higher dimensions.
% Third, thresholding significant latent dimensions (e.g., $|z|>1.96$) is a pragmatic choice; alternative multiple-comparison controls or uncertainty-aware criteria could change interpretability outputs.
% Finally, because a public preprint exists, anonymity cannot be guaranteed even under double-blind review; we therefore focus on full anonymization of the submitted manuscript and supplementary materials.

% Promising directions include evaluating robustness under explicit distribution shifts (new scanners/sites), extending to additional modalities and longitudinal trajectories, improving uncertainty quantification for deviation estimates, and studying how deviation maps relate to downstream clinical endpoints or treatment response.


==> Sections/experimental_setup.tex <==
\paragraph{Data and feature preprocessing}

%We used data from the Alzheimer’s Disease Neuroimaging Initiative (ADNI) dataset \cite{mueller2005ways}. 
For training, we selected 248 cognitively unimpaired (healthy control) subjects with Clinical Dementia Rating (CDR) = 0 and no amyloid pathology. The two input modalities were regional brain volumes from T1-weighted MRI scans and regional Standardized Uptake Value Ratio (SUVR) values from AV45 Amyloid PET scans (Figure 1). Both brain volumes and SUVR values were extracted from 66 cortical (Desikan-Killiany atlas) and 24 subcortical regions. For evaluation, we used a heldout cohort of 48 healthy controls and a disease cohort of 726 amyloid positive AD spectrum (ADS) individuals across: (a) preclinical stage with no symptoms $(CDR = 0, A+) (N = 305)$, (b) $CDR = 0.5 (N = 236)$ and (c) $CDR >= 1 (N = 185)$. 

Each brain ROI was normalised by subtracting the mean and dividing by the standard deviation computed from the healthy control cohort brain regions. We conditioned our model on the age and sex of patients, represented as one-hot encoding vectors, to reduce covariate effects on the MRI and PET features. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Baselines and implementation details} We compared mmSIVAE with (i) Unimodal Soft-Instrospective VAE (SIVAE) \cite{daniel2021soft}(Multimodal VAE (Aim 2B; mmVAE) \cite{kumar_normative_2023}, (ii) unimodal VAE \cite{pinaya_using_2021}, and \textbf{state-of-the-art multimodal VAE models}: mmJSD \cite{sutter2020multimodal}, JMVAE \cite{suzuki2016joint} and MVTCAE \cite{hwang2021multi}. For multimodal methods (mmSIVAE and mmVAE), we compared aggregation techniques (POE, MOE and MOPOE). Unimodal methods (SIVAE and VAE) used a single encoder and decoder and were trained on either a single modality (MRI/amyloid) or both modalities concatenated as a single input. Models mmJSD, JMVAE and MVTCAE were implemented using the open-source Multi-view-AE python package \cite{aguila2023multi}.

We performed grid search over [0.05, 1.0] for $\beta_\text{kl}$ and $\beta_\text{rec}$ and [$\beta_\text{kl}$, 5$\beta_\text{kl}$] for $\beta_\text{neg}$. Following hyperparameter tuning, the final values selected are $\beta_\text{kl} = \beta_\text{kl} = 1$ and $\beta_\text{neg} = 10$. As followed in the SIVAE paper, we set constant $\gamma_r = 10^{-8}$ and s = 1/number of features = 1/90. All models were implemented in Pytorch and trained with Adam for epochs = 500 using learning rate = $10^{-5}$ and batch size = $64$, with latent dimensions in the range [5,10,15,20]. The encoder and decoder networks used 2 fully-connected layers of sizes ${64, 32}$ and ${32, 64}$ respectively.




==> Sections/methods.tex <==
\subsection{Problem setup: multimodal normative modeling}
\label{subsec:setup}

We consider multimodal observations $X=\{x_1,\ldots,x_N\}$ and aim to learn a generative model of a reference (normative) population to quantify subject-specific deviations at test time.
In our application, $x_i$ denotes regional neuroimaging features from modality $i$ (MRI volumes and amyloid PET SUVR), and the reference population comprises cognitively unimpaired, amyloid-negative participants.
We learn the reference distribution using only the normative cohort and derive deviation scores that measure how unlikely an individual is under the learned normative model.

\subsection{Multimodal soft-introspective VAE (mmSIVAE)}
\label{subsec:mmsivae}

\paragraph{Multimodal VAE backbone.}
We parameterize unimodal encoders $q_{\phi_i}(z\mid x_i)$ and a shared latent $z$, together with modality-specific decoders $p_{\theta_i}(x_i\mid z)$.
The multimodal generative model is $p_\theta(X,z)=p(z)\prod_{i=1}^{N}p_{\theta_i}(x_i\mid z)$.
Learning requires a joint approximate posterior $q(z\mid X)$ constructed from the unimodal posteriors (Section~\ref{subsec:aggregation}).
Given $q(z\mid X)$, the corresponding multimodal ELBO is defined in Eq.~\eqref{eq:mv_elbo}.
To reduce confounding effects of covariates, we condition the encoder on age and sex by concatenating their embeddings to the encoder inputs.

\paragraph{Soft-introspective training objective.}
We extend Soft-IntroVAE to the multimodal setting by applying an introspective objective to the joint latent inferred from multimodal observations.
Let $\mathcal{L}_r(X)$ denote the (multimodal) reconstruction term for real inputs and $KL(X)$ the KL divergence between the joint posterior and the prior:
\begin{equation}
\begin{aligned}
\mathcal{L}_r(X)
&=
\mathbb{E}_{q(z \mid X)}
\Big[\sum_{i=1}^{N} \log p_\theta(x_i \mid z)\Big], \\
KL(X)
&=
\mathrm{KL}\!\left(q(z \mid X)\,\|\,p(z)\right).
\end{aligned}
\label{eq:lr_kl_real}
\end{equation}
In our implementation, reconstruction error is measured using mean-squared error (L2).

For generated samples, let $D_\theta(z)$ denote a decoded sample from $z\sim p(z)$ (across modalities).
We define the analogous terms $\mathcal{L}_r(D_\theta(z))$ and $KL(D_\theta(z))$ using the posterior inferred from generated samples.
The mmSIVAE encoder and decoder objectives are:
\begin{equation}
\begin{aligned}
\mathcal{L}_{E_\phi}(X, z)
&=
s\!\cdot\!\Big(\beta_{\mathrm{rec}}\mathcal{L}_r(X)
+\beta_{\mathrm{kl}} KL(X)\Big) \\
&\quad +
\frac{1}{2}\exp\!\Big(
-2s\!\cdot\!\big(
\beta_{\mathrm{rec}}\mathcal{L}_r(D_\theta(z))
+\beta_{\mathrm{neg}} KL(D_\theta(z))
\big)\Big),
\end{aligned}
\label{eq:mmSIVAE_complete_encoder}
\end{equation}

\begin{equation}
\begin{aligned}
\mathcal{L}_{D_\theta}(X, z)
&=
s\!\cdot\!\beta_{\mathrm{rec}}\mathcal{L}_r(X) \\
&\quad +
s\!\cdot\!\Big(
\beta_{\mathrm{kl}} KL(D_\theta(z))
+\gamma_r\,\beta_{\mathrm{rec}}\mathcal{L}_r(D_\theta(z))
\Big).
\end{aligned}
\label{eq:mmSIVAE_complete_decoder}
\end{equation}

Here $\beta_{\mathrm{rec}}$ and $\beta_{\mathrm{kl}}$ control the trade-off between reconstruction fidelity and sample diversity (as in $\beta$-VAE), and $\beta_{\mathrm{neg}}$ controls the repulsion strength for the KL term on generated samples inside the exponential.
Following \cite{daniel2021soft}, $\gamma_r$ downweights the influence of the reconstruction term for generated data in the decoder objective to stabilize early training.
We use a scaling constant $s$ to balance the ELBO and expELBO terms and set $s$ to the inverse of the input dimensionality \cite{daniel2021soft}, preventing the exponential term from vanishing for high-dimensional inputs.

\subsection{Multimodal posterior aggregation via MOPOE}
\label{subsec:aggregation}

A key component in multimodal learning is the construction of $q(z\mid X)$ from unimodal posteriors.
PoE (Eq.~\eqref{eq:poe}) can be dominated by an overconfident modality, whereas MoE (Eq.~\eqref{eq:moe_elbo}) may produce an insufficiently fused joint representation \cite{wu_multimodal_2018,shi2019variational}.
We therefore adopt Mixture-of-Product-of-Experts (MOPOE), which mixes PoE posteriors over subsets of modalities to balance sharpness and robustness.
Let $\mathcal{P}(X)$ denote the set of all non-empty subsets of modalities.
For a subset $S\in\mathcal{P}(X)$, define a PoE posterior
$q_{\mathrm{PoE}}(z\mid X_S)\propto p(z)\prod_{x_i\in X_S}q_{\phi_i}(z\mid x_i)$.
MOPOE is then:
\begin{equation}
q_{\mathrm{MOPOE}}(z\mid X)
=
\frac{1}{|\mathcal{P}(X)|}
\sum_{S\in\mathcal{P}(X)}
q_{\mathrm{PoE}}(z\mid X_S).
\label{eq:mopoe}
\end{equation}
In practice, MOPOE aggregates evidence from modality subsets and yields a shared latent representation that is less sensitive to any single modality while remaining informative for deviation scoring (see Supplement Appendix~B for a proof sketch).

\subsection{Multimodal normative deviation scores}
\label{subsec:deviation}

After fitting the model on the reference population, we quantify deviations for an individual using both latent-space and feature-space statistics.

\paragraph{Latent-space deviation.}
For a subject, we infer a joint latent representation from $q_{\mathrm{MOPOE}}(z\mid X)$ and use the posterior mean $\mu_z$ as the subject embedding.
We fit a multivariate Gaussian to latent means from the reference cohort with mean $\mu_{\mathrm{ref}}$ and covariance $\Sigma_{\mathrm{ref}}$.
The latent deviation score is the Mahalanobis distance:
\begin{equation}
D_{ml}(X)
=
\sqrt{(\mu_z-\mu_{\mathrm{ref}})^\top
\Sigma_{\mathrm{ref}}^{-1}
(\mu_z-\mu_{\mathrm{ref}})}.
\label{eq:dml}
\end{equation}
We additionally compute per-dimension latent $z$-scores relative to the reference distribution to identify significantly deviating latent dimensions.

\paragraph{Feature-space deviation.}
To localize deviations to observed features, we compute modality-wise reconstruction errors and compare them to the distribution of reconstruction errors in the reference cohort.
Let $e(X)=\big[x_1-\hat{x}_1;\ldots;x_N-\hat{x}_N\big]$ denote the concatenated reconstruction-error vector.
We fit a Gaussian to $e(X)$ over the reference cohort with mean $\mu_e$ and covariance $\Sigma_e$ and define the feature-space deviation score:
\begin{equation}
D_{mf}(X)
=
\sqrt{(e(X)-\mu_e)^\top
\Sigma_e^{-1}
(e(X)-\mu_e)}.
\label{eq:dmf}
\end{equation}
Feature-wise $z$-scores of reconstruction errors yield region-level deviation maps.

\subsection{Mapping latent deviations to regional abnormalities}
\label{subsec:interpretability}

To improve interpretability, we map statistically significant latent deviations to regional feature-space deviations.
Let $s_j$ denote the latent $z$-score for dimension $j$ relative to the reference cohort.
We select the set $\mathcal{J}=\{j:\,|s_j|>1.96\}$ of significantly deviating latent dimensions.
We then construct a masked latent vector $\tilde{z}$ that retains only dimensions in $\mathcal{J}$ (setting the remaining dimensions to their reference means), decode $\tilde{z}$ to obtain $\tilde{X}$, and compute region-level deviations from $X-\tilde{X}$.
Finally, to summarize group-level effects across clinical stages, we compute Cohen's $d$ between groups for each region and control for multiple comparisons using FDR correction.


==> Sections/methods_og.tex <==
\section{Proposed methodology}

In this section, we introduce multimodal soft-introspective VAE (mmSIVAE), extending SIVAE (\cite{daniel2021soft}) to the multimodal setting. First, we present the theoretical analysis of mmSIVAE, followed by modeling of the joint latent posterior using the Mixture-of-Product-of-Experts (MOPOE) technique. Next, we discuss how mmSIVAE can be adopted for multimodal normative modeling which includes model training, inference and calculation of subject-level deviations.

\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.9\linewidth]{Figures_tables/mmSIVAE.pdf}
    %\vspace{-10pt}
    \caption{Training flow of mmSIVAE. The ELBO for real samples is optimized for both encoders and decoders, while the encoders also optimize the expELBO to ’push away’ generated samples from the latent space. The decoders optimize the ELBO for the generated samples to 'fool' the encoders.}
    %\vspace{-10pt}
    \label{fig:mmsivae}
\end{figure}

Following Equation \eqref{SIVAE}, the encoder and decoder loss functions for mmSIVAE can be written as:

\vspace{-3mm}
\begin{equation}
\begin{aligned}
& \mathcal{L}_{E_\phi}(X, z)=E L B O(X)-\frac{1}{\alpha} \exp \left(\alpha E L B O\left(D(z)\right)\right) \\
& \mathcal{L}_{D_\theta}(X, z)=E L B O(X)+\gamma E L B O\left(D(z)\right) \label{mmSIVAE}
\end{aligned}
\end{equation}
\vspace{-3mm}

where $X=\left\{x_i \mid i^{th} \text{modality}\right\}$, and $\alpha >= 0$, $\gamma >= 0$ are hyperparameters. $ELBO(X)$ is defined in Equation \eqref{eq:mmELBO}. $ELBO(D(z))$ can be defined similarly, but with $D_\theta(z)_i = p_\theta\left(x_i \mid z\right)$ replacing x in Equation \eqref{eq:mmELBO}. Following $\operatorname{ELBO}(D(z)$ in Equation \ref{eq:mmELBO}, $\operatorname{ELBO}(D(z)$ can be written as: 

\vspace{-3mm}
\begin{equation}
\operatorname{ELBO}(D(z)) \triangleq \mathbb{E}_{q(z \mid X)}\left[\sum_{D_\theta(z)_i \in D} \log p_\theta\left(D_\theta(z)_i \mid z\right)\right]-\operatorname{KL}\left[q_\phi(z \mid D)\| p(z)\right]
\end{equation}
\label{ELBO(D(z)}
\vspace{-3mm}

Equation \eqref{mmSIVAE} represents a min-max game between the encoders and the decoders. The encoders are encouraged, via the ELBO value, to differentiate between real samples (high ELBO) and generated samples (low ELBO), while the decoders aim to generate samples that “fool” the encoders (Figure \ref{fig:mmsivae}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Theoretical analysis}

In this section, we extend the theoretical analysis of SIVAE (\cite{daniel2021soft}) for multimodal data and analyze the Nash equilibrium of the min-max game shown in Equation \eqref{mmSIVAE}. Here, the encoder is represented by the approximate joint posterior distirbution $q=q(z|X)$ and the decoder is represented by $d = p_d(X|z)$. $p_{data}(X)$ represents the data distribution and $p(z)$ denote a prior distribution over the latent variable z. Using the conditional indepence of the modalities and the linearity of the expectation, we can denote $p_d(x_i)=\mathbb{E}_{p(z)}\left[p_d(x_i \mid z)\right]$, which is the distribution of generated samples.

We can further denote $ELBO(X)$ and $ELBO(D(z))$ from Equation \eqref{mmSIVAE} as $W(X; d, q)$ and $W(D; d, q)$ respectively, as shown below. $D$ is the collection of decoders $D = \left\{D_\theta(z)_i \mid i^{th} \text{decoder}\right\}$. 

\vspace{-3mm}
\begin{equation}
\begin{aligned}
ELBO (X) = W(X ; d, q) &\doteq \mathbb{E}_{q(z \mid X)}\left[\sum_{x_i \in X} \log p_d\left(x_i \mid z\right)\right]-K L(q(z \mid X) \| p(z)) \\
ELBO (D(z)) = W(D ; d, q) &\doteq \mathbb{E}_{q(z \mid X)}\left[\sum_{D_\theta(z)_i \in D}\log p_d\left(D_\theta(z)_i \mid z\right)\right]-K L(q(z \mid D) \| p(z))
\end{aligned}
\end{equation}
\vspace{-3mm}

\noindent We consider a nonparametric setting where d and q can be any distribution. For some z, let D(z) be a multimodal sample from $p_d (X \mid z)$ The objective functions for q and d are given by:
\vspace{-3mm}
\begin{equation}
\begin{aligned}
& \mathcal{L}_{E_\phi}(x, z)= [W(X ; q, d)] -\frac{1}{\alpha} \exp \left(\alpha [W(D(z) ; q, d)]\right) \\
& \mathcal{L}_{D_\theta}(x, z)=[W(X ; q, d)] +\gamma E L B O\left([W(D(z) ; q, d)]\right)
\end{aligned}
\end{equation}
\vspace{-3mm}

\noindent The complete mmSIVAE objective functions considers the expectation of the encoder and decoder losses over real ($p_{data}$) and generated ($p_d$) samples.

\vspace{-3mm}
\begin{equation}
\begin{aligned}
& L_q(q, d)=\mathbb{E}_{p_{\text {data }}}[W(X ; q, d)]-\mathbb{E}_{p_d}\left[\alpha^{-1} \exp (\alpha W(X ; q, d))\right], \\
& L_d(q, d)=\mathbb{E}_{p_{\text {data }}}[W(X ; q, d)]+\gamma \mathbb{E}_{p_d}[W(X ; q, d)] \label{complete_mmSIVAE_objective}
\end{aligned}
\end{equation}
\vspace{-3mm}

A Nash equilibrium point $(q^*,d^*)$ satisfies $L_q\left(q^*, d^*\right) \geq L_q\left(q, d^*\right)\quad$ and $\quad L_d\left(q^*, d^*\right) \geq L_d\left(q^*, d\right) \quad \forall q,d.$

Given a $d$, let $q^*(d)$ satisfy $L_q(q^*(d),d) \geq L_q(q,d)$ $\forall$ $q$.

\textbf{Lemma 1:} If $\sum_{i}p_d(x_i) \leq p_{\text {data }}(X)^{\frac{1}{\alpha+1}}$ for all $X$ for which $p_{\text {data }}(X) > 0$, we have that $q^*(d)$ satisfies $q^*(d)(z|X) = p_d(z|X)$, and $W(X;q^*(d),d) = \sum_i \log p_d(x_i)$.

\textbf{Lemma 2}: Let $d^*$ be defined so that $d^* \in \underset{d}{\arg \min }\left\{K L\left(p_{data}(X) \| p_d(X)\right)+\gamma H\left(p_d(X)\right)\right\}$, where $H(\cdot)$ is the Shannon entropy of the generated data samples. If $q^* = p_{d^*}(z \mid x)$, ($q^*, d^*$) is a Nash equilibrium of Equation \eqref{complete_mmSIVAE_objective}.

The proofs of Lemma 1 and 2 are provided in Appendix A.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Modeling of the joint posterior - MOPOE}

In Section 2.3, we discuss the limitations of commonly used techniques POE and MOE for aggregating information from multiple modalities in the latent space. In this work, we adopted a generalization of both MoE and PoE, called Mixture-of-Product-of-Experts (MoPoE) as shown below.

\vspace{-7mm}
\begin{gather}
q_{PoE}(z \mid X_k) \propto \prod_{x_i \in X_k} q(z|x_i) \\
q_{MoPoE}(z|X) = \frac{1}{2^N} \sum_{X_k \in P(X)} q_{PoE}(z|X_k) \\
ELBO_{MOPOE} = \mathbb{E}_{q(z \mid X)}\left[\sum_{x_i \in X} \log p_\theta\left(x_i|z\right)\right]- \operatorname{KL}\left[q_{MoPoE}(z|X),p(z)\right]
\end{gather}
\vspace{-7mm}

Here, $X_k$ denotes a random subset of the N modalities, and $P(X)$ signifies the power set of all N modalities. MoPoE can be viewed as a hierarchical distribution: first, the unimodal posterior approximations for a subset $X_k$ are merged via PoE, followed by the aggregation of subset approximations $q_\phi(z \mid X_k)$ through MoE. This approach leverages the advantages of both MoE and PoE, addressing their respective limitations.

\textbf{Lemma 3}: MoPoE generates a generalized ELBO with PoE and MoE being special cases.

To prove this lemma, first we need to show that $\operatorname{ELBO}_{MoPoE}(X)$ is a valid multimodal ELBO, i.e. $\log p_\theta(x) \geq \operatorname{ELBO}_{MoPoE}(X)$. Next we will show that MOPOE is a generalized case of both POE and MOE. The proofs have been provided in Appendix B.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model training and hyperparameters}

\input{training_algo}

Algorithm 1 shows the detailed training procedure of mmSIVAE. Expanding mmSIVAE's objective function, which is minimized from Equation \ref{mmSIVAE} with the complete set of hyperparameters.

\vspace{-7mm}
\begin{align}
\mathcal{L}_{E_\phi}(X, z) &= s \cdot \left( \beta_{\text{rec}} \mathcal{L}_r(X) + \beta_{\text{kl}} KL(X) \right) 
+ \frac{1}{2} \exp \left( -2s \cdot \left( \beta_{\text{rec}} \mathcal{L}_r(D_\theta(z)) + \beta_{\text{neg}} KL(D_\theta(z)) \right) \right) \label{mmSIVAE_complete_encoder} \\
\mathcal{L}_{D_\theta}(X, z) &= s \cdot \beta_{\text{rec}} \mathcal{L}_r(X) 
+ s \cdot \left( \beta_{\text{kl}} KL(D_\theta(z)) + \gamma_r \cdot \beta_{\text{rec}} \mathcal{L}_r(D_\theta(z)) \right) \label{mmSIVAE_complete_decoder}
\end{align}
\vspace{-7mm}

where $\mathcal{L}_r(X) = \mathbb{E}_{q(z \mid X)}\left[\sum_{x_i \in X} \log p_\theta\left(x_i \mid z\right)\right]$ denotes the summation of reconstruction error of real samples X across the 2 modalities. $KL(X) = \operatorname{KL}\left[q(z \mid X)\| p(z)\right]$ denotes the KL divergence between the joint posterior and prior $p(z)$.

Similarly, $\mathcal{L}_r(D_\theta(z)) = \mathbb{E}_{q(z \mid X)}\left[\sum_{D_\theta(z)_i \in D}\log p_d\left(D_\theta(z)_i \mid z\right)\right]$ denote the summation of the reconstruction error of the generated samples $D(z)$ across the 2 modalities. $KL(D(z)) = KL(q(z \mid D) \| p(z)$ denote the KL divergence between the joint posterior of generated samples $D(z)$ and the prior $p(z)$. 

The hyperparameters $\beta_\text{rec}$ and
$\beta_\text{kl}$ control the balance between inference and sampling quality respectively. When $\beta_\text{rec} > \beta_\text{kl}$, the optimization is focused on good reconstructions, which may lead to less variability in the generated samples, as latent posteriors are allowed to be very different from the prior. When $\beta_\text{rec} < \beta_\text{kl}$, there will be more varied samples, but reconstruction quality will degrade.

Each ELBO term in Equations \ref{mmSIVAE_complete_encoder} and \ref{mmSIVAE_complete_decoder} can be considered as an instance of $\beta_\text{VAE}$ and can have different $\beta_\text{rec}$ and $\beta_\text{kl}$ parameters. However, we set them all to be the same, except for the ELBO inside the exponent in Equation \ref{mmSIVAE_complete_encoder}. For this term, $\beta_\text{kl}$ controls the repulsion force of the posterior for generated samples from the prior. We denote this specific parameter as $\beta_\text{neg}$. 

As reported in the SIVAE paper \cite{daniel2021soft}, the decoder tries to minimize the reconstruction error for generated data, which may slow down convergence, as at the beginning of the optimization the generated samples are of low quality. $\gamma_r$ is a hyperparameter that multiplies only the reconstruction term of the generated data in the ELBO term of the decoder in Equation \ref{mmSIVAE_complete_decoder}. 

Finally, we use a scaling constant s to balance between the ELBO and the expELBO terms in the loss, and we set s to be the inverse of the input dimensions \cite{daniel2021soft}. This scaling constant prevents the expELBO from vanishing for high-dimensional input in Equation \ref{mmSIVAE_complete_encoder}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.9\linewidth]{Figures_tables/latent_deviations.pdf}
    \vspace{-10pt}
    \caption{Normative modeling using multimodal soft-intro VAE (mmSIVAE). Deviations calculated in the latent space using Mahalonobis distance can be used to detect outlier AD patients. The normative performance is evaluated by the likelihood ratio (higher = better).}
    \vspace{-20pt}
    \label{fig:latent_deviations}
\end{figure}

\subsection{Multimodal normative modeling}

mmSIVAE (Figure 1) has separate encoders to encode the 2 modalities into their corresponding latent parameters
(mean and variance). The unimodal latents were aggregated
through the MoPoE approach to estimate the shared latent parameters (joint latent distribution). The shared latents were passed through the modality-specific decoders to reconstruct each modality. The model was first trained to characterize the healthy population cohort. We assumed disease abnormality can be quantified by measuring how AD subjects deviate from the joint space (latent deviations) \cite{lawry_aguila_multi-modal_2023,lawry_aguila_conditional_2022} or from the reconstruction errors of healthy controls (feature-space deviations) \cite{kumar_normative_2023,kumar2024analysing}. During inference, the trained model was applied on the AD cohort to estimate both latent and feature deviations.

\subsubsection*{Patient-specific deviations - latent and feature space}

\textbf{Mahalanobis distance:} To quantify how much AD each subject deviates from the latent distribution of healthy controls, we measured the Mahalanobis distance \cite{lawry2023multi}, which accounts for correlations between latent vectors.

\vspace{-7mm}
\begin{align}
D_{ml} &=\sqrt{(z_j - \mu(z_{norm}))^\top\Sigma(z_{norm})^{-1}(z_j - \mu(z_{norm}))} \label{d_ml}
\end{align}
\vspace{-7mm}

where $z_j \equiv q(z_j|X_j)$ is a sample from the joint posterior distribution for subject $j$. $\mu(z_{norm})$ and $\Sigma(z_{norm})$ represent the mean and covariance of the healthy cohort latent position. We additionally derived a multivariate feature-space deviation index based on the Mahalanobis distance that quantifies how the reconstruction error of an AD subject deviate from the reconstruction errors of controls.

\vspace{-7mm}
\begin{align}
D_{mf} &=\sqrt{(d_j - \mu(d_{norm}))^\top\Sigma(d_{norm})^{-1}(d_j - \mu(d_{norm}))} \label{d_mf}
\end{align}
\vspace{-7mm}

where $d_j = [d^1_j, ...d^i_j, ..d^R_j]$ is the mean squared reconstruction error between original and reconstructed input for subject j and brain region $i = [1, 2,..R]$. $\mu(d_{norm})$ and $\sigma(d_{norm})$ are the mean and covariance of the healthy cohort reconstruction error respectively. 

\textbf{Z-score latent and feature deviations:} To analyze which latent dimensions and brain regions are associated with abnormal deviations due to AD pathology, we calculated both latent space Z-scores $Z_{ml}$ (for each latent dimension) and feature-space Z-scores $Z_{mf}$. $z_{ij}$ and $d_{ij}$ represent the latent values and reconstruction error of test subject j for i-th position respectively. $\mu(z_{ij}^{norm})$ ($\mu(d_{ij}^{norm})$) and $\sigma(z_{ij}^{norm})$ ($\sigma(d_{ij}^{norm})$) are the mean and standard deviations of healthy cohort latent values (reconstruction error) respectively. 

\vspace{-10mm}
\begin{align}
Z_{ml} = \frac{z_{ij} - \mu(z_{ij}^{norm})}{\sigma(z_{ij}^{norm})} \label{z_ml}\\ 
Z_{mf} = \frac{d_{ij} - \mu(d_{ij}^{norm})}{\sigma(d_{ij}^{norm})} \label{z_mf}
\end{align} 


==> Sections/results.tex <==
\section{Results}
\label{sec:results}

We evaluate mmSIVAE on (i) reconstruction fidelity on held-out healthy controls, (ii) separability of deviation scores between healthy controls and AD-spectrum cohorts, (iii) association with cognitive composites, and (iv) interpretability via regional deviation mapping.

\subsection{Reconstruction fidelity on the reference distribution}
\label{subsec:results_recon}

Normative modeling depends on accurately capturing the reference (healthy) distribution; inflated reconstruction error on healthy controls can increase false positives and reduce separation from disease cohorts.
Fig.~\ref{fig:recon_comparison_Aim3} compares reconstruction errors across unimodal and multimodal models.
Across modalities, mmSIVAE yields more faithful reconstructions than VAE baselines, particularly when using multimodal aggregation, indicating improved modeling of the reference distribution.

\subsection{Deviation-score separation and outlier detection}
\label{subsec:results_ood}

\paragraph{Latent-space deviation.}
We first assess separability using the latent Mahalanobis deviation score $D_{ml}$ (Eq.~\eqref{eq:dml}).
Fig.~\ref{fig:latent_deviations} illustrates the deviation-scoring pipeline and the likelihood-ratio-based separation metric.
Table~\ref{tab:latent_sig_ratio_table} summarizes likelihood ratios across latent dimensions and aggregation strategies.
Overall, mmSIVAE with MOPOE achieves the strongest separation between the held-out healthy cohort and the AD-spectrum cohorts, and the best-performing latent dimensionality is consistent with a compact but informative shared representation.

\paragraph{Feature-space deviation.}
We next evaluate the feature-space deviation score $D_{mf}$ (Eq.~\eqref{eq:dmf}), computed from the distribution of reconstruction errors.
Fig.~\ref{fig:feature_mahalanobis_histogram} shows that the deviation-score distributions exhibit clearer separation under mmSIVAE compared to VAE baselines, supporting improved outlier detection in feature space.
Additional quantitative comparisons for feature-space likelihood ratios are provided in the Supplement.

\subsection{Association with cognitive measures}
\label{subsec:results_cognition}

To assess clinical relevance, we compute Pearson correlations between latent deviation $D_{ml}$ and cognitive composite scores.
Table~\ref{tab:cog_correlation_table} reports correlations for memory, executive function, language, and visuospatial abilities, along with statistical tests comparing correlation strength across methods.
Across domains, mmSIVAE demonstrates stronger and more consistent associations with cognitive measures than VAE baselines, suggesting that the learned deviation scores capture clinically meaningful variation beyond group labels.

\subsection{Interpretable deviation mapping}
\label{subsec:results_interp}

\paragraph{Significant latent dimensions.}
We compute latent $z$-scores relative to the reference cohort and identify significantly deviating latent dimensions using $|z|>1.96$.
Fig.~\ref{fig:sig_latent_dimensions} summarizes the distribution of mean deviations across latent dimensions and motivates selecting a sparse subset of dimensions for interpretability.

\paragraph{Regional effect sizes across clinical stages.}
We map significant latent deviations to regional feature deviations (Section~\ref{subsec:interpretability}) and quantify group differences using Cohen's $d$ with FDR correction.
Fig.~\ref{fig:effect_size_interpretability} shows effect-size maps across disease stages for MRI- and PET-derived regional features.
These maps highlight stage-dependent patterns of deviation and provide a region-level interpretation of the learned normative deviations.

